In-Context Learning with Representations: Contextual Generalization of Trained Transformers

In-context learning (ICL) refers to a remarkable capability of pretrained large language models, which can learn a new task given a few examples during inference. However, theoretical understanding of ICL is largely under-explored, particularly whether transformers can be trained to generalize to unseen examples in a prompt, which will require the model to acquire contextual knowledge of the prompt for generalization. This paper investigates the training dynamics of transformers by gradient descent through the lens of non-linear regression tasks. The contextual generalization here can be attained via learning the template function for each task in-context, where all template functions lie in a linear space with $m$ basis functions. We analyze the training dynamics of one-layer multi-head transformers to in-contextly predict unlabeled inputs given partially labeled prompts, where the labels contain Gaussian noise and the number of examples in each prompt are not sufficient to determine the template. Under mild assumptions, we show that the training loss for a one-layer multi-head transformer converges linearly to a global minimum. Moreover, the transformer effectively learns to perform ridge regression over the basis functions. To our knowledge, this study is the first provable demonstration that transformers can learn contextual (i.e., template) information to generalize to both unseen examples and tasks when prompts contain only a small number of query-answer pairs.

==> setup_.tex <==
\section{Problem Setup} \label{sec:setup}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{In-context learning with representation.}
We consider ICL of  regression with unknown representation, similar to the setup introduced in \citet{guo2023transformers}. To begin, let  $f: \R^d\rightarrow\R^m $
 be a fixed representation map that $f(\vx)=(f_1(\vx),\cdots,f_m(\vx))^\top$ for any $\vx \in \R^d$. The map $f$ can be quite general, which can be regarded as a feature extractor that will be learned by the transformer. We assume that each ICL task corresponds to a map $\vlambda^\top f(\cdot)$ that lies in the linear span of those $m$ basis functions in $f(\cdot)$, where $\vlambda$ is generated according to the distribution $\mathcal{D}_{\vlambda}$. Thus, for each ICL instance, the (noisy) label of an input $\vv_k$ ($\forall k\in[K]$) is given as 
% \begin{equation} \label{eq:ICL_clean} 
% y = f_{\vlambda}(\vx) =  \langle \vlambda, f(\vx) \rangle = \sum_{i=1}^m \lambda_i f_i (\vx), \qquad  \vlambda\sim \mathcal{P}_{\vlambda},
% \end{equation}
\begin{equation} \label{eq:ICL} 
\quad y_k =  \vlambda^\top(f(\vv_k)+\veps_k), \qquad  \vlambda\sim \mathcal{D}_{\vlambda},\quad \veps_k\overset{i.i.d.}{\sim}\mathcal{N}(0,\tau\mI_m)
\end{equation}
 where 
 %$\mathcal{P}_{\vlambda}$ is the  distribution of $\vlambda$, and 
 $\tau>0$ is the noise level. 
 
 The goal of ICL is to form predictions on query $\vx_{\mathsf{query}}$ given in-context labels of the form \eqref{eq:ICL} on a few inputs, known as {\em prompts}. In this paper, we use $\voc$ to denote the {\em dictionary} set that contains all $K$ unit-norm {\em distinct} tokens, i.e., $\voc\coloneqq\left\{\vv_1,\cdots,\vv_K\right\}\subset \R^{d}$ with each token $\norm{\vv_k}_2=1$.
%given a length-$K$ dictionary of {\em distinct} tokens $\voc\coloneqq\left\{\vv_1,\cdots,\vv_K\right\}\subset \R^{d}$ of unit-norms, i.e., $\norm{\vv_k}_2=1$, 
We assume that each prompt $P=P_{\vlambda}$ provides the first $N$ tokens (with $N \ll K$) and their labels, 
%   \begin{equation}\label{eq:prompt}
%P=P(\vlambda)\coloneqq(\vv_1,y_1,\cdots,\vv_N,y_N), 
%\end{equation}
and is embedded in the following matrix
\begin{equation}\label{eq:embedding}
  \mE^P  \coloneqq
  \begin{pmatrix}
    \vv_1 & \vv_2 & \cdots & \vv_N\\
    y_1 & y_2 & \cdots & y_N
  \end{pmatrix} \coloneqq   \begin{pmatrix} 
  \promptmtrx \\
  \vy^{\top}
   \end{pmatrix} 
  \in \mathbb{R}^{(d+1)\times N},
  \end{equation}
where 
\begin{equation}\label{eq:prompt_token}
\promptmtrx\coloneqq(\vv_1,\cdots,\vv_N)\in\R^{d\times N}
\end{equation}
 is the collection of prompt tokens, and $\vy\coloneqq\left(y_1,\cdots, y_N\right)^\top$ is the prompt label. 
Given the prompt as the input, the transformer predicts the labels for all the $K$ tokens $y_1,\cdots,y_K$ in the dictionary set. 
 
 
  

\begin{figure}[t]
    \centering
 \includegraphics[width=0.8\textwidth]{figs/model.png} 
 %\vspace{-0.25in}
    \caption{The structure of a one-layer transformer with multi-head softmax attention.}
    \label{fig:structure}
\end{figure}

\paragraph{Transformer architecture.} 
We adopt a one-layer transformer with multi-head softmax attention \citep{chen2024training} --- illustrated in \Cref{fig:structure} --- to predict the labels of all the tokens in the dictionary $\voc$, where $H$ is the number of heads. Denote the query embedding as
\begin{equation}\label{eq:padding}
    \mE^Q\coloneqq
    \begin{pmatrix}
      \vv_{N+1} &\vv_{N+2} &\cdots &\vv_K\\
      0 &0 &\cdots &0
    \end{pmatrix}\in\R^{(d+1)\times (K-N)},
\end{equation}
and denote the embedding of both the prompt and the query as $\mE\coloneqq(\mE^P , \mE^Q )\in\R^{(d+1)\times K}$.
We define the output of each transformer head as
\begin{equation} \label{eq:head}
\text{head}_h(\mE)\coloneqq\mW_h^{\mathsf{V}} \mE^P \cdot \sm\left((\mE^{P})^\top(\mW_h^{\mathsf{K}})^\top\mW_h^\mathsf{Q} {\mE} \right),\quad h\in[H],
\end{equation}
where $\mW_h^\mathsf{Q} \in\R^{d_{\text{e}} \times (d+1)} $, $\mW_h^{\mathsf{K}} \in\R^{ d_{\text{e}} \times (d+1)}$, and $\mW_h^{\mathsf{V}}\in\R^{K\times (d+1)}$ are the query, key, and value matrices, respectively, 
%for queries, keys, and values, respectively, 
and the softmax is applied column-wisely, i.e., given a vector input $\vx$, the $i$-th entry of $\sm(\vx)$ is given by $e^{x_i}/\sum_{j}e^{x_j}$.
The attention map of the transformer $\transformer(\mE)$ is defined as
\begin{equation}\label{eq:transformer_structure}
    \transformer(\mE)\coloneqq \mW^\mathsf{O}
    \begin{pmatrix}
        \text{head}_1(\mE) \\
        \vdots \\
        \text{head}_H(\mE)
    \end{pmatrix} \in \mathbb{R}^{K\times K}, 
\end{equation}
where $\mW^\mathsf{O}$ is the output matrix. Following recent theoretical literature to streamline analysis \citep{huang2023context,nichani2024transformers,deora2023optimization,chen2024training}, we assume that the embedding matrices take the following forms: 
\begin{subequations}
\begin{align}
\mW^\mathsf{O}  \coloneqq\left(\mI_K,\cdots,\mI_K\right) & \in\R^{K\times HK},\quad \mW_h^{\mathsf{V}}\coloneqq(\vzero,\vw_h)\in\R^{K\times (d+1)}, \label{eq:W_O_W_V} \\
 (\mW_h^{\mathsf{K}})^\top\mW_h^\mathsf{Q} & =
\begin{pmatrix}
    \mQ_h & \vzero \\
    \vzero & 0
\end{pmatrix}\in\R^{(d+1)\times(d+1)},\quad \forall h\in[H], \label{eq:W_KQ}
\end{align}
\end{subequations}
where $\vw_h=(w_{h,1},\cdots,w_{h,K})^\top\in\R^K$ and $\mQ_h\in R^{d\times d}$ are trainable parameters for all $h\in[H]$.  

The prediction of the labels  is provided by the diagonal entries of $ \transformer(\mE)$, which we denote by $\vypred=(\widehat y_1, \cdots, \widehat y_K)\in\R^K$.
%denote the diagonal of $\transformer(\mE)$.
Note that $\widehat y_k$ takes the following form under our parameter specification:
\begin{equation}\label{eq:y_predict}
    \forall k\in[K]:\qquad \widehat y_k=\Big\langle\vy,\sum_{h=1}^H w_{h,k}\,\sm(\promptmtrx^\top\mQ_h\vv_k)\Big\rangle.
\end{equation}
 
%Our transformer structure is shown in Figure~\ref{fig:structure}.

%\yl{we may need to use wrapfigure for Fig. 1 to save space}

%We stress that the multi-head mechanism is essential in this context. In Section~\ref{sec:interpretation} we argue that a transformer with only one attention is not be able to gain in-context ability in our problem setting.
\paragraph{Training via GD.} 
Let $\vtheta=\{\mQ_h,\vw_h\}_{h=1}^H$ denote all trainable parameters of $\transformer$. Let $\epsfull\coloneqq (\veps_1,\cdots,\veps_K)\in\R^{m\times K}$ denote the noise matrix. Given training data over ICL instances, the goal of training is to predict labels $y_k$ for all $\vv_k\in\voc$. Specifically, we train the transformer using gradient descent (GD) by optimizing the following mean-squared population loss:
\begin{equation}\label{eq:loss}
  \LL(\vtheta)\coloneqq\frac{1}{2}\EE_{\vlambda,\epsfull}\left[\frac{1}{K}\sum_{k=1}^K \left(\widehat y_k-y_k\right)^2\right].
\end{equation}
%where $y_k\coloneqq f_\lambda(\vv_k)$ is the label of the $k$-th token, $k\in[K]$. 
We apply different learning rates  $\eta_Q,\eta_w>0$ for updating $\left\{\mQ_h\right\}_{h=1}^H$ and $\left\{\vw_h\right\}_{h=1}^H$, respectively, i.e., at the $t$-th ($t\geq 1$) step, we have
\begin{align} \label{eq:original_GD}
    \forall h\in[H]:\quad\mQ_h^{(t)}=\mQ_h^{(t-1)}-\eta_Q\nabla_{\mQ_h} \LL(\vtheta^{(t-1)}),\quad \vw_h^{(t)}=\vw_h^{(t-1)}-\eta_w\nabla_{\vw_h} \LL(\vtheta^{(t-1)}),
\end{align}
where $\vtheta^{(t)}=\{\mQ_h^{(t)},\vw_h^{(t)}\}_{h=1}^H$ is the parameter at the $t$-th step.
 

\paragraph{Inference time.} At inference time, given a prompt $P=P_{\vlambda}$ with $N$ examples, where \textit{$\vlambda$ may not be in the support of the generation distribution $\mathcal{D}_{\vlambda}$}, the transformer applies the pretrained parameters and predicts the labels of all $K$ tokens without further parameter updating.

==> theory_.tex <==
\section{Theoretical Analysis} \label{sec:theory}

\subsection{Training time convergence}\label{sec:theory_training}

In this section, we show that the training loss $\LL$ converges to its minimum value at a linear rate during training, i.e., the function gap
\begin{equation}\label{eq:gap}
    \Delta^{(t)}\coloneqq\LL(\vtheta^{(t)})-\inf_{\vtheta}\LL\rightarrow 0,\quad t\rightarrow \infty
\end{equation}
at a linear rate, under some appropriate assumptions.


\paragraph{Key assumptions.} We first state our technical assumptions. The first assumption is on the distribution $\mathcal{D}_{\vlambda}$ for generating the coefficient vector $\vlambda$ of the representation maps.
\begin{asmp}[Assumption on distribution $\mathcal{D}_{\vlambda}$]\label{asmp:lambda_dist}
  We assume that in \eqref{eq:ICL} each entry $\lambda_i$ is drawn independently  and satisfies $\EE[\lambda_i]=0$ and $\EE[\lambda_i^2]=1$ for all $i\in[m]$.
\end{asmp}


To proceed, we introduce the following notation:
\begin{equation}\label{eq:Z}
\mZ\coloneqq \left( f(\vv_1) \cdots f(\vv_N)\right)\in\R^{m\times N},\quad
\bar{\mZ}\coloneqq\left(\mZ^\top\mZ+m\tau\mI_N\right)^{1/2}\in\R^{N\times N}, 
\;\; \bar f_{\max}\coloneqq \max_{i\in[N]}\norm{\bar\vz_i}_2,
\end{equation}
where $\bar\vz_i$ is the $i$-th column vector of $\bar\mZ$ for $i\in[N]$. We further define  $\mC_k^{(t)}$ ($k\in[K]$, $t\in\NN_+$) and $\mB_k^{(t)}$ as follows:
\begin{equation}\label{eq:matrix_C_B}
    \mC_k^{(t)}\coloneqq \sm(\promptmtrx^\top\mQ_1^{(t)}\vv_k,\cdots,\promptmtrx^\top\mQ_H^{(t)}\vv_k)\in\R^{N\times H},\qquad \mB_k^{(t)}=\bar\mZ\mC_k^{(t)}\in\R^{N\times H}.
\end{equation}

     
  
% --------------------------------------------------------------------------------------------------

To guarantee the convergence, we require the initialization of the parameters  $\vtheta^{(0)}$ satisfies the following condition.
\begin{asmp}[Assumption on initialization]\label{asmp:gamma}
    %There exists $\gamma>0$ such that
   For all $k\in[K]$, $\mB_k^{(0)}$ has full row rank. 
\end{asmp}



\paragraph{Choice of learning rates.} Define 
\begin{equation}\label{eq:eigen_0}
\zeta_0\coloneqq\min_{k\in[K]}\left\{\lambda_{\min}\left(\mB_k^{(0)}\mB_k^{(0)\top}\right)\right\},
\end{equation}
where $\Delta^{(0)}$ is the initial function gap (c.f.~\eqref{eq:gap}). Assumption~\ref{asmp:gamma} indicates that $\zeta_0>0$.
Let $\gamma$ be any positive constant that satisfies 
    \begin{equation}\label{eq:condition}
        \gamma\geq \zeta_0^{-5/4}\left(\frac{128\sqrt{2}}{\sqrt{2}-1}\norm{\bar\mZ}_2^2 \sqrt{H}\bar f_{\max}K^{3/2}\Delta^{(0)}\right)^{1/2}.
    \end{equation}
    We set the learning rates as
    \begin{equation}\label{eq:choice_lr}
        \eta_Q\leq 1/ L \quad\text{and} \quad \eta_w=\gamma^2\eta_Q,
    \end{equation}
    where\footnote{We leave a tighter, but more complicated, expression of $L$ in the appendix (cf. \eqref{eq:L_tight}) in the appendix and present a simplified form in the main paper for readability.}
    \begin{align} 
            % \bar L^2&= 2\left(\frac{1}{K}\left(2\gamma\norm{\bar\mZ}_2^2 \left(2\gamma H\bar\alpha+\norm{\mA}_2\right)\right)^2+\frac{\gamma^4}{K^2} H^2\norm{\bar\mZ}_2^4\right)\\
            % &\quad + 8\gamma \bar f_{\max}\norm{\bar\mZ}_2 \cdot\max\left\{1, (2\sqrt{K}\bar\alpha )^2\right\}\left[(\bar\alpha\gamma H)^2+4N\left(\bar\alpha\gamma H+\norm{\mA}_2\right)^2\right],
            \textstyle L^2&\textstyle=\left(8\sqrt{2}H\sqrt{K}\frac{\norm{\bar\mZ}_2^2}{\zeta_0}\sqrt{\Delta^{(0)}}+1+\frac{\norm{\mZ^\top\Zfull}_2}{m\tau}\right)^2\norm{\bar\mZ}_2^4\cdot\left(\frac{8}{K}\gamma^2+\frac{4096}{\gamma\zeta_0^2}K^2 N\Delta^{(0)}\right)\nonumber \\
            &\textstyle \qquad+2H^2\norm{\bar\mZ}_2^4\left(\frac{\gamma^4}{K^2}+\frac{16384}{\gamma \zeta_0^4}K^3\norm{\bar\mZ}_2^2\left(\Delta^{(0)}\right)^2\right).
 \label{eq:smoothness_const_bar_L}
        % \bar\alpha&= \sqrt{2K}\frac{4\norm{\bar\mZ}_2}{\gamma\zeta_0}\sqrt{\bar\LL (\vtheta^{(0)})-\inf_{\vtheta}\bar\LL(\vtheta)},\\
        %\mA&= \left(\mZ^\top\mZ+m\tau\mI_N\right)^{-1}\left(\mZ^\top\Zfull + \left(m\tau\mI_N,\vzero\right)\right)\in\R^{N\times K}.
    \end{align}

\paragraph{Theoretical guarantee.} Now we are ready to state our first main result, regarding the training dynamic of the transformer.
\begin{thm}[Training time convergence]\label{thm:rate_under}
    Suppose Assumptions~\ref{asmp:lambda_dist},~\ref{asmp:gamma} hold. We let $\vw_k^{(0)}=\vzero$ and set the learning rates as in \eqref{eq:choice_lr}. Then we have
    \begin{equation}\label{eq:rate_under}
        \LL(\vtheta^{(t)})-\inf_{\vtheta}\LL(\vtheta)\leq \left(1-\frac{\eta_w\zeta_0}{2K}\right)^t\left(\LL(\vtheta^{(0)})-\inf_{\vtheta}\LL(\vtheta)\right),\quad \forall t\in\NN.
    \end{equation} 
\end{thm}
\begin{proof}
See Appendix~\ref{sec_app:proof_rate_under}. 
 \end{proof}
 
 Before we provide more interpretations of Theorem~\ref{thm:rate_under}, let us turn back to examine the initialization condition in Assumption~\ref{asmp:gamma}. 
We require the following mild assumption on $\promptmtrx$ to ensure our parameter initialization has good properties.
\begin{asmp}[Assumption on $\promptmtrx$]\label{asmp:init}
    There exists one row vector $\vx=(x_1,\cdots,x_N)^\top$ of the prompt token matrix $\,\promptmtrx$ (cf.~\eqref{eq:prompt_token}) such that $x_i\ne x_j$, $\forall i\ne j$.  
\end{asmp}

Assumption~\ref{asmp:init} implies that $\voc$ has distinct tokens, i.e., $\vv_j\ne\vv_k$ when $j\ne k$. It is worth noting that Assumption~\ref{asmp:init} is the only assumption we have on the dictionary $\voc$. In comparison, all other theoretical works in Table~\ref{tb:comparison} impose somewhat unrealistic assumptions on $\voc$. For example, 
\citet{huang2023context,li2023transformers,nichani2024transformers} assume that the tokens are pairwise orthogonal, which is restrictive since it implies that the dictionary size $K$ should be no larger than the token dimension $d$, whereas in practice it is often the case that $K\gg d$~\citep{reid2024gemini,touvron2023llama}. In addition, \citet{chen2024training,zhang2023trained,wu2023many} assume that each token is independently sampled from some Gaussian distribution, which also does not align with practical scenarios where tokens are from a fixed dictionary and there often exist (strong) correlations between different tokens. 
 
 
The following proposition states that when the number of heads exceeds the number of prompts, i.e. $H\geq N$, we can guarantee that Assumption~\ref{asmp:gamma} holds with probability 1 by simply initializing $\{\mQ_h\}_{h=1}^H$ using Gaussian distribution.
\begin{prop}[Initialization of $\{\mQ_h\}_{h=1}^H$]\label{prop:init}
    Suppose Assumptions~\ref{asmp:lambda_dist},~\ref{asmp:init} hold and $H\geq N$. For any fixed $\beta>0$, let $\mQ_h^{(0)}(i,j)\overset{i.i.d.}{\sim}\mathcal{N}(0,\beta^2)$, then Assumption~\ref{asmp:gamma} holds almost surely.
\end{prop}
\begin{proof}
See Appendix~\ref{sec_app:proof_prop_init}.
\end{proof}

Theorem~\ref{thm:rate_under}, together with Proposition~\ref{prop:init}, shows that the training loss converges to its minimum value at a linear rate, under mild assumptions of the task coefficients and token dictionary. This gives the \textit{first} convergence result for transformers with multi-head softmax attention trained using GD to perform ICL tasks (see Table~\ref{tb:comparison}). Our convergence guarantee \eqref{eq:rate_under} also indicates that the convergence speed decreases as the size $K$ of the dictionary or the number $H$ of attention heads increases, which is intuitive because training with a larger vocabulary size or number of parameters is more challenging. However, a small $H$ will limit the expressive power of the model (see Section~\ref{sec:interpretation} for detailed discussion), and we require $H\geq N$ to guarantee Assumption~\ref{asmp:gamma} holds, as stated in Proposition~\ref{prop:init}.








\subsection{Inference time performance}\label{sec:inference}  

We now move to examine the inference time performance, where the  coefficient vector $\vlambda$ corresponding to the inference task may  not drawn from $\mathcal{D}_{\vlambda}$. In fact, we only assume that the coefficient vector $\vlambda$ at inference time is bounded as in the following assumption.
\begin{asmp}[Boundedness of $\vlambda$ at inference time]\label{asmp:boundedness}
    We assume that at inference time $\norm{\vlambda}_2\leq B$ for some $B>0$.
\end{asmp} 



For notational simplicity, let $\mZ^Q\in\R^{m\times (K-N)}$ denote
\begin{equation}\label{eq:Z^Q}
    \mZ^Q \coloneqq(f(\vv_{N+1}),\cdots,f(\vv_{K}))\in\R^{m\times (K-N)}.
\end{equation}  
The following theorem characterizes the performance guarantee of the transformer's output $\vypred$ (after sufficient training) at the inference time. 
\begin{thm}[Inference time performance]\label{thm:inference_under}
  Let  $\widehat\vlambda$ be the solution to the following ridge regression problem:
\begin{equation}\label{eq:ridge_regression}
\textstyle \widehat\vlambda\coloneqq\argmin_{\vlambda}\left\{\frac{1}{2N}\sum_{i=1}^N( y_i-\vlambda^\top f(\vv_i))^2+\frac{m\tau}{2N}\norm{\vlambda}_2^2\right\}.
\end{equation}
Under the assumptions in Theorem~\ref{thm:rate_under}, for any $\varepsilon>0$ and $\delta\in(0,1)$, if the number of training iterates $T$ satisfies
    \begin{equation}\label{eq:iteration_complexity_under}
        %\begin{split}
 \textstyle           T\geq \frac{\log\bigg(B^2\Delta^{(0)}\left(\norm{\mZ}_2+\sqrt{\tau}\left(2\sqrt{N\log(1/\delta)}+2\log(1/\delta)+N\right)^{1/2}\right)^2\Big /\left(m\tau\varepsilon\right)\bigg)}{\log\left(1/\left(1-\frac{\eta_w\zeta_0}{2K}\right)\right)},    
        %     \\
        % &\asymp \frac{4K\log\bigg(\frac{B\sqrt{2K(\Delta^{(t)}(\vtheta))\left(\norm{\mZ}_2+\sqrt{\tau}\left(2\sqrt{N\log(1/\delta)}+2\log(1/\delta)+N\right)^{1/2}\right)}}{\sqrt{m}\varepsilon}\bigg)}{\eta_w\zeta_0},
        %\end{split}
    \end{equation}
    then given any prompt $P$ that satisfies Assumption~\ref{asmp:boundedness} at the inference time, with probability at least $1-\delta$, the output of the transformer $\vypred$ satisfies
    \begin{equation}\label{eq:esp_acc_under}
\frac{1}{2K}\norm{\vypred-\vylimit}_2^2\leq \varepsilon, \qquad \text{with}\quad \vylimit\coloneqq \begin{pmatrix}
        \vy \\
        \left(\mZ^Q\right)^\top \widehat\vlambda
    \end{pmatrix}.
    \end{equation} 
\end{thm}

\begin{proof}
See Appendix~\ref{sec_app:proof_inference_under}.
\end{proof} 

In Theorem~\ref{thm:inference_under}, \eqref{eq:esp_acc_under} shows that after training, the transformer learns to output the given labels of the first $N$ tokens in each prompt, and more importantly, predicts the labels of the rest $K-N$ tokens by implementing the ridge regression given in \eqref{eq:ridge_regression}.  
Note that \citet{akyurek2022learning} studied the expressive power of transformers on the linear regression task and showed by construction that transformers can represent the closed-form ridge regression solution. Interestingly, here we show from an optimization perspective that transformers can in fact be trained to do so.

\paragraph{Generalization capabilities of the pretrained transformer.} Theorem~\ref{thm:inference_under} captures two generalization capabilities that the pretrained transformer can have. 
\begin{enumerate}[i)]
\item {\em Contextual generalization to unseen examples:} Theorem~\ref{thm:inference_under} suggests that %the pretrained transformer, without knowing the function map $f$ is able to attain the performance of the regression regression in \cref{eq:ridge_regression}, solving which requires the knowledge of $f$. This implies that 
the transformer exploits the {\em inherent contextual} information (to be further discussed in \Cref{sec:interpretation}) of the function template in the given prompt, and can further use such information to predict the unseen tokens. 
\item {\em Generalization to unseen tasks:} Theorem~\ref{thm:inference_under} also suggests that the pretrained transformer can generalize to a function map corresponding to any $\vlambda\in \R^{m}$ at the inference time (albeit satisfying Assumption~\ref{asmp:boundedness}), which is not necessarily sampled from the support of its training distribution $\mathcal{D}_{\vlambda}$. 
\end{enumerate}
%See Figure~\ref{fig:1_layer_loss},\ref{fig:4_layer_loss} Section~\ref{sec:exp} for empirical validation of these two generalization capabilities.

%Theorem~\ref{thm:inference_under} shows that when the labels in the prompt is not sufficient to determine the template that generates the prompt, the transformer the transformer choose the template by performing ridge regression. This sheds light on how transformers predict the labels of unseen tokens in the prompt. Crucially, this finding cannot be reflected by other works that study the optimization of in-context learning of transformers with softmax attention~

We note that the contextual generalization that the transformer has here is different in nature from the prediction ability shown in previous works on ICL \citep{huang2023context,chen2024training,li2024training,nichani2024transformers}. Those work focuses on a setting where each prompt contains a good portion of tokens similar to the query token, allowing the transformer to {\em directly} use the label of the corresponding answers from the prompt as the prediction. However, in practical scenarios, prompts often contain only partial information, and our analysis sheds lights on explaining how transformers generalize to unseen examples by leveraging ridge regression to infer the underlying template. 

%how good is transformer's choice of the underdetermined template? 
 
\paragraph{How does the representation dimension affect the performance?}
Beyond the above discovery, several questions are yet to be explored. For instance, while
we demonstrate that transformers can be trained to implement ridge regression, how good is the performance of the ridge regression itself? What is the best choice of ridge regression we could expect? How close is the transformer's choice to the best possible choice? We address these questions as follows.
 
Given any prompt $P$ at inference time, since there is no label information about the rest $K-N$ tokens, the best prediction we could hope for from the transformer shall be
   \begin{equation}\label{eq:best_prediction}
       \widehat\vy^{\text{best}}\coloneqq \begin{pmatrix}
        \vy \\
        \left(\mZ^Q\right)^\top \widehat\vlambda_\tau
    \end{pmatrix},
    \end{equation}\label{eq:minimize_norm}
    where $\mZ^Q$ is defined in \eqref{eq:Z^Q}, and $\widehat\vlambda_\tau$ satisfies:
    \begin{equation}\label{eq:regression_noisy}
        \textstyle \widehat\vlambda_\tau\coloneqq\argmin_{\vlambda}\E_{\tilde{\veps}}\left[\frac{1}{2N}\sum_{i=1}^N(y_i-\vlambda^\top \left(f(\vv_i)+\veps_i\right))^2\right].
    \end{equation}
    In other words, we hope the transformer outputs the given $N$ labels as they are. For the rest $K-N$ labels, the best we could hope for is that the transformer estimates the coefficient vector $\vlambda$ by solving the above regression problem to obtain $\widehat\vlambda_\tau$, and predict the $k$-th label by $\widehat\vlambda_\tau^\top f(\vv_k)$ for $k=N+1,\cdots,K$. 
    Note that \eqref{eq:regression_noisy} is equivalent to the following ridge regression problem (see Lemma~\ref{lm:equivalence} in the appendix for its derivation):    \begin{equation}\label{eq:ridge_regression_best}
    \textstyle \widehat\vlambda_\tau=\argmin_{\vlambda}\left\{\frac{1}{2N}\sum_{i=1}^N(y_i-\vlambda^\top f(\vv_i))^2+\frac{\tau}{2}\norm{\vlambda}_2^2\right\}.
    \end{equation}
    The only difference between the two ridge regression problems \eqref{eq:ridge_regression} and \eqref{eq:ridge_regression_best} is the coefficient of the regularization term. This indicates that at the training time, the transformer learns to implement ridge regression to predict the labels of the rest $K-N$ tokens, assuming the noise level is given by $\frac{m}{N}\tau$.
    This observation also reflects how the sequence length $N$ affects the transformer's preference for choosing templates and its performance at inference time:
\begin{itemize} 
    \item The closer $m$ is to $N$, the closer the transformer's choice of templates is to the best possible choice, and the better the transformer's prediction will be;
    \item When $N<m$, the transformer tends to underfit by choosing a $\vlambda$ with small $\ell_2$-norm;
    \item When $N>m$, the transformer tends to overfit since it underestimates the noise level and  in turn captures noise in the prediction.
\end{itemize}
 

\subsection{Further interpretation}\label{sec:interpretation} 

We provide more interpretation on our results, which may lead to useful insights into the ICL ability of the transformer. 

\paragraph{How does the transformer gain ICL ability with representations?} 
Intuitively speaking, our pretrained transformer gains in-context ability by extracting and memorizing some ``inherent information'' of all basic function maps $f_i$ ($i\in[m]$) during the training. Such information allows it to infer the coefficient vector $\vlambda$ from the provided labels in each prompt and calculate the inner product $\inner{\vlambda}{f(\vv_k)}$ to compute $y_{k}$ given any token $\vv_{k}\in\voc$ at inference time.  
To be more specific, the ``inherent information'' of all basic tasks could be described by the $N$-by-$K$ matrix $\mA$ defined as follows (see also \eqref{eq:matrix_A}):
$$\mA\coloneqq \left(\mZ^\top\mZ+m\tau\mI_N\right)^{-1}\left(\mZ^\top\Zfull + \left(m\tau\mI_N,\vzero\right)\right)\in\R^{N\times K},$$
where $\Zfull\coloneqq (f(\vv_1),\cdots,f(\vv_K))=(\mZ,\mZ^Q)\in\R^{m\times K}$.
% \begin{align}\label{eq:AZ}
% \mA\coloneqq\left(\mZ^\top\mZ+m\tau\mI_N\right)^{-1}\left(\mZ^\top\Zfull + \left(m\tau\mI_N,\vzero\right)\right), \,\,\text{where} \,\,\Zfull\coloneqq (f(\vv_1),\cdots,f(\vv_K))\in\R^{m\times K}.
% \end{align}
%
During training, the transformer learns to approximate $\mA_{:,k}$ by $\sum_{h=1}^H w_{h,k}\sm(\promptmtrx^\top\mQ_h\vv_k)$ for each $k\in[K]$. 

To further elaborate, we take a closer look at the special case when the labels do not contain any noise, i.e., $\tau=0$, and $N\geq m$. In this case, $\mA$ becomes $\mZ^\dag\Zfull$, and given any prompt $P=P_{\vlambda}$, the coefficient vector $\vlambda$ could be uniquely determined from the provided token-label pairs in the prompt. It is straightforward to verify that the label of each token $\vv_k$ could be represented by the inner product of the given label vector $\vy$ and the $k$-th column of $\mZ^\dag\Zfull$, i.e.,
\begin{equation}\label{eq:label_representation}
  y_k=\inner{\vy}{\mZ^\dag\Zfull_{:,k}}.
\end{equation}
Comparing the above equation with \eqref{eq:y_predict}, it can be seen that in order to gain the in-context ability, the transformer needs to learn an approximation of $ \mZ^\dag\Zfull_{:,k}$ by $\sum_{h=1}^H w_{h,k}\sm(\promptmtrx^\top\mQ_h\vv_k)$ for each $k\in[K]$.

More generally, in the proof of Theorem~\ref{thm:inference_under}, we show that
\begin{equation}\label{eq:y_limit}
    \vylimit_k=\inner{\vy}{\mA_{:,k}},
\end{equation}
comparing which with \eqref{eq:y_predict} suggests that a small training error implies that $\sum_{h=1}^H w_{h,k}\sm(\promptmtrx^\top\mQ_h\vv_k)$ is close to $\mA_{:,k}$. In fact, this is the necessary and sufficient condition for the training loss to be small. A rigorous argument is provided in Lemma~\ref{lm:loss_reform_under}.
 

\paragraph{The importance of multi-head attention mechanism.} Multi-head attention mechanism is essential in our setting. In fact, it is generally impossible to train a shallow transformer with only one attention head to succeed in the ICL task considered in our paper. This is because, as we have discussed above, the key for the transformer is to approximate  $\mA_{:,k}$ by $\sum_{h=1}^H w_{h,k}\sm(\promptmtrx^\top\mQ_h\vv_k)$ for each $k\in[K]$. If $H=1$, the transformer could not approximate each $\mA_{:,k}$ by $w_{1,k}\sm(\promptmtrx^\top\mQ_1\vv_k)$ in general since the entries of the latter vector are either all positive or all negative. In addition, Proposition~\ref{prop:init} indicates that when $H\geq N$, the weights of the transformer with a simple initialization method satisfy our desired property that is crucial to guarantee the fast linear convergence. However, \eqref{eq:rate_under} implies that we should not set $H$ to be too large, since larger $H$ yields slower convergence rate.  

%Below we give our proof sketch.

 
